Fisheye Consistency: Keeping Data in Synch in a Georeplicated World

Over the last thirty years, numerous consistency conditions for replicated data have been proposed and implemented. Popular examples of such conditions include linearizability (or atomicity), sequential consistency, causal consistency, and eventual consistency. These consistency conditions are usually defined independently from the computing entities (nodes) that manipulate the replicated data; i.e., they do not take into account how computing entities might be linked to one another, or geographically distributed. To address this lack, as a first contribution, this paper introduces the notion of proximity graph between computing nodes. If two nodes are connected in this graph, their operations must satisfy a strong consistency condition, while the operations invoked by other nodes are allowed to satisfy a weaker condition. The second contribution is the use of such a graph to provide a generic approach to the hybridization of data consistency conditions into the same system. We illustrate this approach on sequential consistency and causal consistency, and present a model in which all data operations are causally consistent, while operations by neighboring processes in the proximity graph are sequentially consistent. The third contribution of the paper is the design and the proof of a distributed algorithm based on this proximity graph, which combines sequential consistency and causal consistency (the resulting condition is called fisheye consistency). In doing so the paper not only extends the domain of consistency conditions, but provides a generic provably correct solution of direct relevance to modern georeplicated systems.

==> proofSCCConsistency_flawed.tex <==
%% \commentFT{Consider a history $H$ created by Algorithm~\ref{alg:SC:CC:consistency-prot}, we want to show that $H$ fulfills the conditions of $\mathcal{G}$-fisheye
%%  (SC,CC)-consistency defined in Section~\ref{sec:fish-cons-pair}.\\
%% \\
%% Because the (SC,CC)-broadcast used in Algorithm~\ref{alg:SC:CC:consistency-prot} insures causal order on its messages, this translate to a causal order $\leadsto_{H}$ on the operation of $H$ while respecting the \emph{read from} relation $\overset{\text{rf}}{\rightarrow}$, and the process order relation $\overset{\text{po}}{\rightarrow}$.
%% \\
%% We now want to show we can construct an order $\leadstostar_{H,\mathcal{G}}$ from $\leadsto_{H}$ that fulfills the conditions of Section~\ref{sec:fish-cons-pair}. The idea is to use a similar construction as the one that shows that the WW constraints (total order on write operations) is sufficient to ensure sequential consistency: recursively add edges to $\leadsto_{H}$ to fulfill the conditions on $\leadstostar_{H,\mathcal{G}}$, while showing that the graph remains acyclic (it's an order), and legal (explaining what legal means for an relation on read-write operations). That is where I think we should relax our condition on total order of $\leadstostar_{H,\mathcal{G}}|(\{p,q\})$ to write operations only, and handle read operations afterwards.}

%\newcommand{\opwrite}{\text{op}_{\mathit{write}}}
%\newcommand{\opread}{\text{op}_{\mathit{read}}}

\newcommand{\opwrite}{w}
\newcommand{\opread}{r}
\newcommand{\rfrel}{\overset{\mathit{rf}}{\rightarrow}}
\newcommand{\porel}{\overset{\mathit{po}}{\rightarrow}}

For readability, we denote in the following $\opread_p(X,v)$ the read operation invoked by process $p$ on object $X$ that returns a value $v$ ($X.\text{read} \rightarrow v$), and $\opwrite_p(X,v)$ the write operation of value $v$ on object $X$ invoked by process $p$ ($X.\text{write}(v)$). We may omit the name of the process when not needed.

Let us consider a history $\widehat{H}=(H,\porel_H)$ that captures an execution of Algorithm~\ref{alg:SC:CC:consistency-prot}, i.e., $\porel_H$ captures the sequence of operations in each process (process order, $po$ for short). We construct the causal order $\leadsto_H$ required by the definition of Section~\ref{sec:fish-cons-pair} in the following, classical, manner:
\begin{itemize}
\item We connect each read operation $\opread_p(X,v)=X.\text{read} \rightarrow v$ invoked by process $p$ (with $v\neq \bot$, the initial value) to the write operation $\opwrite(X,v)=X.\text{write}(v)$ that generated the \textsc{write}$(X,v)$ message carrying the value $v$ to $p$ (line~\ref{line:allocating:v:to:vx} in Algorithm~\ref{alg:SC:CC:consistency-prot}). In other word we add an edge $\langle\opwrite(X,v) \overset{\mathit{rf}}{\rightarrow} \opread_p(X,v)\rangle$ to $\porel_H$ (with $\opwrite$ and $\opread_p$ as described above) for each read operation $\opread_p(X,v) \in H$ that does not return the initial value $\bot$. We connect initial read operations $\opread(X,\bot)$ to an $\bot$ element that we add to $H$.

We call these additional relations \emph{read-from links} (noted $\rfrel$).
\item We take $\leadsto_H$ to be the transitive closure of the resulting relation.
\end{itemize}

$\leadsto_H$ is acyclic, as assuming otherwise would imply at least one of the \textsc{write}$(X,v)$ messages was received before it was sent. $\leadsto_H$ is therefore an order. We now need to show $\leadsto_H$ is a causal order in the sense of the definition of Section~\ref{sec:causal-consistency}, i.e., that the result of each read operation $\opread(X,v)$ is the value of the latest write $\opwrite(X,v)$ that occurred before $\opread(X,v)$ in $\leadsto_H$ (said differently, that no read returns an overwritten value).

\begin{lemma}\label{lemma:leadstoH:causal}
  $\leadsto_H$ is a causal order.
\end{lemma}

\begin{proofL}\renewcommand{\toto}{lemma:leadstoH:causal}
We show this by contradiction. We assume without loss of generality that all values written are distinct. Let us consider $\opwrite_p(X,v)$ and $\opread_q(X,v)$ so that $\opwrite_p(X,v) \rfrel \opread_q(X,v)$, which implies $\opwrite_p(X,v) \leadsto_H \opread_q(X,v)$. Let us assume there exists a second write operation $\opwrite_r(X,v')\neq \opwrite_p(X,v)$ on the same object, so that
\begin{equation}
 \opwrite_p(X,v) \leadsto_H \opwrite_r(X,v') \leadsto_H \opread_q(X,v)
\end{equation}
\noindent (illustrated in Figure~\ref{fig:leadstoHcausal}).
%
$\opwrite_p(X,v) \leadsto_H \opwrite_r(X,v')$ means we can find a sequence of operations $op_i \in H$ so that
\begin{equation}
  \opwrite_p(X,v) \rightarrow_0 op_0 ... \rightarrow_i op_i \rightarrow_{i+1} ... \rightarrow_k \opwrite_r(X,v')
\end{equation}
\noindent with $\rightarrow_i \in \{\porel_H,\rfrel\}, \forall i\in [1,k]$. The semantics of $\porel_H$ and $\rfrel$ means we can construct a sequence of causally related (SC,CC)-broadcast messages $m_i \in M$ between the messages that are toco\_broadcast by the operations $\opwrite_p(X,v)$ and $\opwrite_r(X,v')$, which we note $\textsc{write}_p(X,v)$ and $\textsc{write}_r(X,v')$ respectively:
\begin{equation}
  \textsc{write}_p(X,v) = m_0 \leadsto_M m_1 ... \leadsto_M m_i \leadsto_M ... \leadsto_M m_{k'} = \textsc{write}_r(X,v')
\end{equation}
\noindent where $\leadsto_M$ is the message causal order introduced in Section~\ref{sec:mathcalg-fisheye-sc}. We conclude that $\textsc{write}_p(X,v) \leadsto_M \textsc{write}_r(X,v')$, i.e., that $\textsc{write}_p(X,v)$ belongs to the causal past of $\textsc{write}_r(X,v')$, and hence that $q$ in Figure~\ref{fig:leadstoHcausal} toco-delivers $\textsc{write}_r(X,v')$ after $\textsc{write}_p(X,v)$.

% comment that same reasoning with remaining operation, with distinction between on same process (q=r), or involves rf relationship, in which case use the blocking behaviour of write operations, so assignment occured of v' arrived (i) after that of v but before read operation, which contradicts the fact that read reads value wriiten by write


\begin{figure}[tbh]
\centering
\usetikzlibrary{calc}
\begin{tikzpicture}[node distance=0.9cm]
  \renewcommand{\makeoplabel}[1]{}
  \renewcommand{\writesyntax}[2]{$w_{\processid}(#1,#2)$}
  \renewcommand{\readsyntax}[2]{$r_{\processid}(#1,#2)$}

  \ProcessWithId{p}{$p$}{6}{%
    \writeOp{X}{v}{0.5}{2.0}{}
  }
  \ProcessWithId{q}{$q$}{6}{%
    \readOp{X}{v}{4.5}{6.0}{}
  }
  \ProcessWithId{r}{$r$}{6}{%
    \writeOp{X}{v'}{2.5}{4.0}{}
  }

  \procmessage{p}{1.25}{q}{5.25}{$\rfrel$}{bend right=2}
  \procmessage{p}{1.25}{r}{2.5}{$\leadsto_H$}{bend right=0,dashed}
  \procmessage{r}{4   }{q}{5.25}{$\leadsto_H$}{bend right=2,dashed}

\end{tikzpicture}
\caption{Proving that $\leadsto_H$ is causal by contradiction}
\label{fig:leadstoHcausal}
\end{figure}

We now want to show that $\textsc{write}_r(X,v')$ is toco-delivered by $q$ before $q$ executes $\opread_q(X,v)$. We can apply the same reasoning as above to $\opwrite_r(X,v') \leadsto_H \opread_q(X,v)$, yielding another sequence of operations $op'_i \in H$:
\begin{equation}
  \opwrite_r(X,v') \rightarrow'_0 op'_0 ... \rightarrow'_i op'_i \rightarrow'_{i+1} ... \rightarrow'_{k''} \opread_q(X,v)
\end{equation}
\noindent with $\rightarrow'_i \in \{\porel_H,\rfrel\}$. Because $\opread_q(X,v)$ does not generate any (SC,CC)-broadcast message, we need to distinguish the case where all $op'_i$ relations correspond to the process order $\porel_H$ (i.e., $op'_i = \porel_H, \forall i$). In this case, $r=q$, and the blocking behavior of $X$.\func{write}() (line~\ref{line:pi:waits} of Algorithm~\ref{alg:SC:CC:consistency-prot}), insures that $\textsc{write}_r(X,v')$ is toco-delivered by $q$ before executing $\opread_q(X,v)$. If at least one $op'_i$ corresponds to the read-from relation, we can consider the latest one in the sequence, which will denote the toco-delivery of a $\textsc{write}_z(Y,w)$ message by $q$, with $\textsc{write}_r(X,v') \leadsto_M \textsc{write}_z(Y,w)$. From the causality of the (SC,CC)-broadcast, we also conclude that $\textsc{write}_r(X,v')$ is toco-delivered by $q$ before executing $\opread_q(X,v)$.

Because q toco-delivers $\textsc{write}_p(X,v)$ before $\textsc{write}_r(X,v')$, and toco-delivers $\textsc{write}_r(X,v')$ before it executes $\opread_q(X,v)$, we conclude that the value $v$ of $v_x$ is overwritten by $v'$ at line~\ref{line:allocating:v:to:vx} of Algorithm~\ref{alg:SC:CC:consistency-prot}, and that $\opread_q(X,v)$ does not return $v$, contradicting our assumption that $\opwrite_p(X,v) \rfrel \opread_q(X,v)$, and concluding our proof that $\leadsto_H$ is a causal order.
\end{proofL}

\newcommand{\leadmoon}{\overset{\leftmoon}{\leadsto}}
\newcommand{\leadsmallstar}{\overset{\medstar}{\leadsto}}

\newcommand{\leadmooninc}[1]{\leadmoon_H^{\raisebox{-0.3em}{$\scriptstyle #1$}}}
\newcommand{\leadsmallstarinc}[1]{\leadsmallstar_H^{\raisebox{-0.3em}{$\scriptstyle #1$}}}
\newcommand{\leadstostarinc}[1]{\leadstostar_H^{\raisebox{-0.3em}{$\scriptstyle #1$}}}

\newcommand{\tocorel}{\overset{ww}{\rightarrow}}

To construct $\leadstostar_{H,\mathcal{G}}$, as required by the definition of (SC,CC)-consistency (Section~\ref{sec:fish-cons-pair}), we first order the write operations of neighboring processes in the proximity graph $\mathcal{G}$. We do so by constructing an intermediary order $\leadmoon_H$ from $\leadsto_H$ as follows:
\begin{itemize}
\item
We add an edge $\opwrite_p(X,v) \tocorel \opwrite_q(Y,w)$ to $\leadsto_H$ for each pair of write operations $\opwrite_p(X,v)$ and $\opwrite_q(Y,w)$ in $H$ such that:
\begin{itemize}
\item $(p,q)\in E_{\mathcal{G}}$ (i.e., $p$ and $q$ are connected in $\mathcal{G}$);
\item $\opwrite_p(X,v)$ and $\opwrite_q(Y,w)$ are not ordered in $\leadsto_H$;
\item The broadcast message $\textsc{write}_p(X,v)$ of $\opwrite_p(X,v)$ has been toco-delivered before the broadcast message $\textsc{write}_p(Y,w)$ of $\opwrite_q(Y,w)$ by all processes.
\end{itemize}

We call these additional edges \emph{ww links} (noted $\tocorel$).
\item We take $\leadmoon_H$ to be the recursive closure of the relation we obtain.
\end{itemize}

$\leadmoon_H$ is acyclic, as assuming otherwise would imply that the underlying (SC,CC)-broadcast violates causality. Because of the $\mathcal{G}$-delivery order and termination of the toco-broadcast (Section~\ref{sec:mathcalg-fisheye-sc}), we know all pairs of $\textsc{write}_p(X,v)$ and $\textsc{write}_p(Y,w)$ messages with $(p,q)\in E_{\mathcal{G}}$ as defined above are toco-delivered in the same order by all processes. This insures that all write operations of neighboring processes in $\mathcal{G}$ are ordered in $\leadmoon_H$.

We need to show that $\leadmoon_H$ remains a causal order, i.e., that no read in $\leadmoon_H$ returns an overwritten value.

\begin{lemma}\label{lemma:leadmoon:causal}
  $\leadmoon_H$ is a causal order.
\end{lemma}

\begin{proofL}\renewcommand{\toto}{lemma:leadmoon:causal}
We extend the original causal order  $\leadsto_M$ on the messages of an (SC,CC)-broadcast execution with the following order $\leadsto_M^{\mathcal{G}}$:

\noindent $m_1 \leadsto_M^{\mathcal{G}} m_2$ if
\begin{itemize}
\item $m_1 \leadsto_M m_2$ ; or
\item $m_1$ was sent by $p$, $m_2$ by $q$, $(p,q)\in E_{\mathcal{G}}$, and $m_1$ is toco-delivered before $m_2$ by all processes; or
\item there exists a message $m_3$ so that $m_1 \leadsto_M^{\mathcal{G}} m_3$ and $m_3 \leadsto_M^{\mathcal{G}} m_2$.
\end{itemize}
$\leadsto_M^{\mathcal{G}}$ captures the order imposed by an execution of an (SC,CC)-broadcast on its messages. The proof is then identical to that of Lemma~\ref{lemma:leadstoH:causal}, except that we use the order $\leadsto_M^{\mathcal{G}}$, instead of $\leadsto_M$.
\end{proofL}

\newcommand{\rwrel}{\overset{rw}{\rightarrow}}

$\leadmoon_H$ imposes a local WW (write-write) constraint~\cite{MRZ1995,R13-Dist-alg} on the write operations of neighboring process in the proximity graph $\mathcal{G}$. To construct $\leadstostar_{H,\mathcal{G}}$ from $\leadmoon_H$, we now need to order the read operations of processes connected in $\mathcal{G}$. We do so in two steps by extending the technique presented in~\cite{MRZ1995}. The first steps insures that the orders we construct remain causal, by ``protecting'' the read-from relation $\rfrel$. The second step orders the remaining reads that did not get ordered in the first step.

The first step works as follows: We construct a sequence of orders $\leadsmallstarinc{i}$, starting from $\leadmoon_H = \leadsmallstarinc{0}$, by repeatedly executing the following construction:
\begin{itemize}
\item We select a pair of (read,write) operations $\opread_p(X,v)$ and $\opwrite_q(Y,w)$ in $H$ such that:
\begin{itemize}
\item $(p,q)\in E_{\mathcal{G}}$ (i.e., $p$ and $q$ are connected in $\mathcal{G}$);
\item $\opread_p(X,v)$ and $\opwrite_q(Y,w)$ are not ordered in $\leadsmallstarinc{i}$;
\item $\opwrite_q(Y,w)$ is ordered in $\leadsmallstarinc{i}$ after the write operation $\opwrite_r(X,v)$ from which $\opread_p(X,v)$ reads its value, i.e., we have $\opwrite_r(X,v) \rfrel \opread_p(X,v)$ and $\opwrite_r(X,v) \leadsmallstarinc{i} \opwrite_q(Y,w)$.
\end{itemize}
\item We add an edge $\opread_p(X,v) \rwrel \opwrite_q(Y,w)$ to $\leadsmallstarinc{i}$. We call this additional edge a \emph{rw link} (noted $\rwrel$, Figure~\ref{fig:constructing:rwrel}).
\item We take $\leadsmallstarinc{i+1}$ to be the recursive closure of the resulting relation.
\end{itemize}

%\nice{a diagram to illustrate what we do above.}
\noindent We repeat the above step until there is no more pair of (read,write) operations $\opread_p(X,v)$ and $\opwrite_q(Y,w)$ that meet the above conditions. We take $\leadsmallstar_H$ to be the final relation obtained.

\newcommand{\relation}[5]{%
  \draw (#1) edge [-latex,#4] node [auto] {\scriptsize #2} #5 (#3);
}

\begin{figure}[tbh]
\centering
\usetikzlibrary{calc}
\usetikzlibrary{snakes}
\begin{tikzpicture}[node distance=2cm]
  \node (w1)               {$\opwrite_r(X,v)$} ;
  \node (r1) [right of=w1] {$\opread_p(X,v)$ } ;
  \node (w2) [right of=r1] {$\opwrite_q(Y,w)$} ;


  \relation{w1}{$\mathit{rf}$}{r1}{}{};
%  \relation{r1}{$\medstar$   }{w2}{snake=snake}{node [below right] {\scriptsize $H$} };
  \relation{r1}{$\mathit{rw}$   }{w2}{dashed}{};
  \relation{w1}{$\leadsmallstarinc{i}$}{w2}{bend right=-30}{};

  %\draw (r1) edge [-latex] node [auto] {\scriptsize $\medstar$} (w2);

\end{tikzpicture}
\caption{Constructing $\leadsmallstarinc{i+1}$ from $\leadsmallstarinc{i}$ by adding an $\rwrel$ edge}
\label{fig:constructing:rwrel}
\end{figure}

By construction, each $\leadsmallstarinc{i}$ is acyclic (we only consider pairs not ordered in $\leadsmallstarinc{i-1}$). Each of them is therefore an order. Each $\leadsmallstarinc{i}$ is also causal (no read returns an overwritten value), as shown by the following lemma.

\begin{lemma}\label{lemma:leadsmallstarinc:is:causal}
  $\forall i$, $\leadsmallstarinc{i}$ is causal.
\end{lemma}

\begin{proofL}\renewcommand{\toto}{lemma:leadsmallstarinc:is:causal}
This is shown by contradiction. If we consider the first edge $\opread_p(X,v) \rwrel \opwrite_q(Y,w)$ to break the causality between $\leadsmallstarinc{i}$ in $\leadsmallstarinc{i+1}$ for some $i$, then because $\opwrite_r(X,v)$ covers $\opread_p(X,v)$ in $\leadsmallstarinc{i}$ (as $\leadsmallstarinc{i}$ is causal), and because the path $\opwrite_r(X,v) \rfrel \opread_p(X,v) \rwrel \opwrite_q(Y,w)$ is doubled in $\leadsmallstarinc{i+1}$ by $\opwrite_r(X,v) \leadsmallstarinc{i} \opwrite_q(Y,w)$ (Figure~\ref{fig:constructing:rwrel}), then we conclude that $\leadsmallstarinc{i}$ was not causal in the first place, contradicting our assumption.
\end{proofL}

\newcommand{\rrwrel}{\overset{\filledstar}{\rightarrow}}

As a result, $\leadsmallstar_H$ is therefore causal. $\leadsmallstar_H$ does not, however, fully order all the operations of processes connected in $\mathcal{G}$. Hence, the second and final step to obtain $\leadstostar_{H,\mathcal{G}}$ adds these missing edges, which always involve at least one read operation (since all write operations of neighboring nodes are ordered by ww links in $\leadmoon_H$). In a way similar to the above technique, we construct a sequence $\leadstostarinc{i}$ starting from $\leadsmallstar_H = \leadstostarinc{0}$, by repeatedly executing the following construction:
\begin{itemize}
\item We select a pair of (read,write) operations $\opread_p(X,v)$ and $\opwrite_q(Y,w)$ in $H$ such that:
\begin{itemize}
\item $(p,q)\in E_{\mathcal{G}}$ (i.e., $p$ and $q$ are connected in $\mathcal{G}$);
\item $\opread_p(X,v)$ and $\opwrite_q(Y,w)$ are not ordered in $\leadstostarinc{i}$;
\end{itemize}
\item We add an edge $\opread_p(X,v) \rrwrel \opwrite_q(Y,w)$ to $\leadstostarinc{i}$. We call this additional edge a \emph{r-rw link} (noted $\rrwrel$).
\item We take $\leadstostarinc{i+1}$ to be the recursive closure of the resulting relation.
\end{itemize}

\noindent We repeat the above step until there is no more pair of (read,write) operations $\opread_p(X,v)$ and $\opwrite_q(Y,w)$ that meet the above conditions. We take $\leadstostar_{H,\mathcal{G}}$ to be the final relation obtained.

As above, each $\leadstostarinc{i}$ is acyclic. We show it is causal.

\begin{lemma}\label{lemma:leadstostarinc:is:causal}
    $\forall i$, $\leadstostarinc{i}$ is causal.
\end{lemma}

\begin{proofL}\renewcommand{\toto}{lemma:leadstostarinc:is:causal}
  We show this by contradiction. Consider the first $\opread_p(X,v) \rrwrel \opwrite_q(Y,w)$ to break the causality in $\leadstostarinc{i+1}$, while $\leadstostarinc{i}$ is causal. This means $\leadstostarinc{i+1}$ contains the pattern on Figure~\ref{fig:leadstostarinc:causal}.

\begin{figure}[tbh]
\centering
\usetikzlibrary{calc}
\usetikzlibrary{snakes}
\begin{tikzpicture}[node distance=2cm,scale=1.5]
  \node (w1) at (1,0)      {$\opwrite_1(Z,z)$} ;
  \node (r1) at (3,0)      {$\opread_1(Z,z)$ } ;
  \node (w2) at (2,-1.5)      {$\opwrite_2(Z,z')$} ;

  \relation{w1}{$\mathit{rf}$}{r1}{}{};
  \relation{w1}{$\leadstostarinc{i+1}$}{w2}{dashed,bend right=30}{};
  \relation{w2}{$\leadstostarinc{i+1}$}{r1}{dashed,bend right=30}{};

  %\draw (r1) edge [-latex] node [auto] {\scriptsize $\medstar$} (w2);

\end{tikzpicture}
\caption{Assuming $\leadstostarinc{i+1}$ is not causal}
\label{fig:leadstostarinc:causal}
\end{figure}

Because $\leadstostarinc{i}$ is causal, at least one of the two paths marked $\leadstostarinc{i+1}$ in Figure~\ref{fig:leadstostarinc:causal} contains $\opread_p(X,v) \rrwrel \opwrite_q(Y,w)$. If we assume $\opread_p(X,v) \rrwrel \opwrite_q(Y,w)$ is only present in the path $\opwrite_1(Z,z) \leadstostarinc{i+1} \opwrite_2(Z,z')$ on the left, we have the situation shown on Figure~\ref{fig:leftcase}. This case implies that $\opwrite_q(Y,w)
\leadstostarinc{i} \opread_1(Z,z)$. Because $\leadstostarinc{i}$ is causal by assumption, this implies $\opwrite_q(Y,w) \leadstostarinc{i} \opwrite_1(Z,z)$, and by transitivity we have $\opwrite_q(Y,w) \leadstostarinc{i} \opread_p(X,v)$. This contradicts the construction of $\leadstostarinc{i+1}$, which implies that $\opwrite_q(Y,w)$ and $\opread_p(X,v)$ were not ordered in $\leadstostarinc{i}$.

\begin{figure}[tbh]
\centering
\usetikzlibrary{calc}
\usetikzlibrary{snakes}
\begin{tikzpicture}[node distance=2cm,scale=1.5]
  \node (w1) at (1,0)        {$\opwrite_1(Z,z)$} ;
  \node (rp) at (1,-0.75)    {$\opread_p(X,v)$}  ;
  \node (wq) at (2,-1.5) {$\opwrite_q(Y,w)$} ;
  \node (r1) at (5,0)        {$\opread_1(Z,z)$ } ;
  \node (w2) at (4,-1.5)     {$\opwrite_2(Z,z')$} ;

  \relation{w1}{$\mathit{rf}$}{r1}{}{};
%  \relation{w1}{$\leadstostarinc{i+1}$}{w2}{dashed,bend right=30}{};
  \relation{w1}{$\leadstostarinc{i}$}{rp}{dashed}{};
  \relation{rp}{$\rrwrel$}{wq}{bend right=20}{};
  \relation{wq}{$\leadstostarinc{i}$}{w2}{dashed}{};
  \relation{w2}{$\leadstostarinc{i}$}{r1}{dashed,bend right=30}{};

  %\draw (r1) edge [-latex] node [auto] {\scriptsize $\medstar$} (w2);

\end{tikzpicture}
\caption{Assuming $\opread_p(X,v) \rrwrel \opwrite_q(Y,w)$ is only present in the path $\opwrite_1(Z,z) \leadstostarinc{i+1} \opwrite_2(Z,z')$}
\label{fig:leftcase}
\end{figure}

Assuming $\opread_p(X,v) \rrwrel \opwrite_q(Y,w)$ is present in the path $\opwrite_2(Z,z') \leadstostarinc{i+1} \opread_1(Z,z)$ on the right of Figure~\ref{fig:leadstostarinc:causal} leads to the same contradiction. This applies whether or not $\opread_p(X,v) \rrwrel \opwrite_q(Y,w)$ is present in $\opwrite_1(Z,z) \leadstostarinc{i+1} \opwrite_2(Z,z')$, thus covering all cases, and concluding the proof.
\end{proofL}

\algoimplemeentscccconst*

\begin{proofT}\renewcommand{\toto}{theo:proof-that-algorithm}
The order $\leadstostar_{H,\mathcal{G}}$ we have just constructed fulfills the conditions required by the definition of $\mathcal{G}$-fisheye (SC,CC)-consistency (Section~\ref{sec:fish-cons-pair}):
\begin{itemize}
\item by construction $\leadstostar_{H,\mathcal{G}}$ subsumes $\leadsto_H$ ($\leadsto_H\;\subseteq\; \leadstostar_{H,\mathcal{G}}$);
\item because $\leadstostar_{H,\mathcal{G}}$ also subsumes any of the orders $\leadsmallstarinc{i}$ and $\leadstostarinc{i}$ introduced earlier, any pair of operations invoked by processes $p$,$q$ that are neighbors in $\mathcal{G}$ are ordered in $\leadstostar_{H,\mathcal{G}}$; i.e., $\mbox{$(\leadstostar_{H,\mathcal{G}})$}|\{p,q\}$ is a total order.
\end{itemize}

To finish the proof, we choose, for each process $p_i$, $\widehat{S}_i$ as one of the topological sorts of $\mbox{$(\leadstostar_{H,\mathcal{G}})$}|(p_i+W)$, following the approach of \cite{MRZ1995,R13-Dist-alg}. $\widehat{S}_i$ is sequential by construction. Because $\leadstostar_{H,\mathcal{G}}$ is causal, $\widehat{S}_i$ is legal. Because $\leadstostar_{H,\mathcal{G}}$ respects $\porel_H$, $\widehat{S}_i$ is equivalent to $\widehat{H}{|(p_i+W)}$. Finally, $\widehat{S}_i$ respects $\mbox{$(\leadstostar_{H,\mathcal{G}})$}|(p_i+W)$ by construction.
\end{proofT}

% final steps: we need to order reads. We do so by pushing them as close as possible to their read-from: before all writes whose WRITE messages ordered after that of their read-from. We take recursive closure

% or should it be all writes ordered in \leadmoon_H after their read from write

% not done yet tough: problem of remaining reads and writes : need to show that adding arbitrary links OK. No cycle (by definition). Is this still causal: case of read--write and read--read


%This can be done

% might be useful later

%% we first construct a sequence of intermediary orders $\leadmooninc{i}$ that incrementally order the write operations of processes $p$ and $q$ connected in $\mathcal{G}$. Starting from $\leadmooninc{0}=\leadsto_H$, we construct $\leadmooninc{i+1}$ from $\leadmooninc{i}$ as follows:
%% \begin{itemize}
%% \item We select a pair of write operations $\opwrite_p(X,v)$ and $\opwrite_q(Y,w)$ in $H$ such that
%%   \begin{itemize}
%%   \item $(p,q)\in E_{\mathcal{G}}$ (i.e., $p$ and $q$ are connection in $\mathcal{G}$);
%%   \item $\opwrite_p(X,v)$ and $\opwrite_q(Y,w)$ are not ordered in $\leadmooninc{i}$.
%%   \end{itemize}
%% \item we arbitrarily order the two write relations by adding a relation $\opwrite_p(X,v) \leadsto_{\mathcal{G}}^{i+1} \opwrite_q(Y,w)$ to $\leadmooninc{i}$;
%% \item we take the recursive closure of the resulting relation, which yields $\leadmooninc{i+1}$.
%% \end{itemize}

